Field of Groves: An Energy-Efficient Random Forest

Machine Learning (ML) algorithms, like Convolutional Neural Networks (CNN), Support Vector Machines (SVM), etc. have become widespread and can achieve high statistical performance. However their accuracy decreases significantly in energy-constrained mobile and embedded systems space, where all computations need to be completed under a tight energy budget. In this work, we present a field of groves (FoG) implementation of random forests (RF) that achieves an accuracy comparable to CNNs and SVMs under tight energy budgets. Evaluation of the FoG shows that at comparable accuracy it consumes ~1.48x, ~24x, ~2.5x, and ~34.7x lower energy per classification compared to conventional RF, SVM_RBF , MLP, and CNN, respectively. FoG is ~6.5x less energy efficient than SVM_LR, but achieves 18% higher accuracy on average across all considered datasets.

==> Makefile <==
LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf -jobname=./out/main
# -pvc specifies if "continuous build" is enabled
CONTINUOUS=-pvc

MAIN=ms

SOURCES=$(MAIN).tex Makefile
FIGURES := $(shell find figures/* images/* -type f)

all: $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	mkdir -p out
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk
	rm -rf out

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all



==> background.tex <==
\section{Background}
\label{sec:background}
%% Subsections
\input{machine-learning-applications}
\input{machine-learning-algos}

==> custom_comms.tex <==
\usepackage{listings} % coding environment (used to show verilog codes)

% Put custom commands here

\makeatletter
% ==========================================
% Define custom commands:

% Align individual rows:
% Usage: \al{l}{foo}
\newcommand*{\al}[2]{\multicolumn{1}{#1}{#2}}

%% Making a box around text
\newcommand{\boxaround}[2]{
  \fbox{\begin{minipage}{#1}{#2}\end{minipage}
}

% This is a Zebra code listing (creates neat ``zebra''-like
% lines with numberings. You can define your own colors
% (modify the code_params.tex)
\newcommand\realnumberstyle[1]{#1}
\newcommand{\zebra}[3]{%
  {\realnumberstyle{#3}}%
  \begingroup
    \lst@basicstyle
    \ifodd\value{lstnumber}%
        \color{#1}%
    \else
        \color{#2}%
    \fi
    \rlap{%
        \hspace*{\lst@numbersep}%
        \color@block{\linewidth}{\ht\strutbox}{\dp\strutbox}%
    }%
  \endgroup
}

% This one is for making spaces around the wrapfigures
% sometimes when the text is short, the wrapfigure will
% try to make everything after itself change its size.
% use \makespace to fix it
\newcommand{\makespace} {
  \par
  \loop
  \ifnum\c@WF@wrappedlines > 1
  \hspace*{1sp}\newline
  \advance\c@WF@wrappedlines by -1
  \repeat
  \par
}


%-------------------------------------------------------------------------
% Extra definitions
%-------------------------------------------------------------------------
% If you would like to get rid of some text, but still have it for future:
% Just put the text that you would like to hide into \ignore{your text}
\def\ignore#1{}
% \newcommand{\ignore}[1]{}

% This is a fixme request. In case of collaboration, this thing will emphasize
% the text and put a FIXME: keyword
% \newcommand{\fixme}[1] {
%  \textbf{\textcolor{red}{[ FIXME: #1 ]}}
% }
\newcommand{\fixme}[1] {
  \todo[backgroundcolor=red!50!white,inline,author=FIXME]{#1}
}

% These are the todo requests
\newcommand{\noteforme}[1] {
  \textbf{\textcolor{blue}{[ NOTE FOR MYSELF: #1 ]}}
}
\newcommand{\todoBlue}[1] {
  \todo[backgroundcolor=blue!20!white,inline,author=TODO]{#1}
}
\newcommand{\todoRed}[1] {
  \todo[backgroundcolor=red!20!white,inline,author=TODO]{#1}
}
\newcommand{\todoGreen}[1] {
  \todo[backgroundcolor=green!20!white,inline,author=TODO]{#1}
}
\newcommand{\todoYellow}[1] {
  \todo[backgroundcolor=yellow!20!white,inline,author=TODO]{#1}
}

% Create tabs
\newcommand{\tab} {
  \hspace{.02\textwidth}
}

% End of commands definition
% ==========================================
\makeatother

% ==========================================
% Define code styles:

% Before defining the verilog code listing, let's fix the referencing
% Use matchrangestart=t as an argument to the lslisting to enable
\makeatletter
\lst@Key{matchrangestart}{f}{\lstKV@SetIf{#1}\lst@ifmatchrangestart} % Define matchrangestart
% Add matchrangestart test to the SkipToFirst:
\def\lst@SkipToFirst{%
    \lst@ifmatchrangestart\c@lstnumber=\numexpr-1+\lst@firstline\fi
    \ifnum \lst@lineno<\lst@firstline
           \def\lst@next{%
                \lst@BeginDropInput\lst@Pmode
                \lst@Let{13}\lst@MSkipToFirst
                \lst@Let{10}\lst@MSkipToFirst}%
           \expandafter\lst@next
    \else
        \expandafter\lst@BOLGobble
    \fi}%
\makeatother

% Verilog styling with Zebra
\lstdefinestyle{custom_verilog}{
  basicstyle=\footnotesize\ttfamily,
  belowcaptionskip=0.1\baselineskip,
  breaklines=true,
  captionpos=t,
  commentstyle=\color{green!60!black},
  deletekeywords={...},
  % Note that @ sign is better to use as an escape character
  % but in Verilog it is already reserved:
  escapeinside={^}{^},
  frame=L,
  identifierstyle=\color{black},
  keywordstyle=\bfseries\color{blue},
  language=Verilog,
  morecomment={
    [s][\color{red}]{/*!}{*}
  },
  morekeywords={
    *,
    % Data type definitions:
    bit,
    electrical,
    logic,
    longint,
    shortint,
    shortreal,
    typedef,
    wreal,
    ...,
    % extra constructs:
    interface,
    endinterface,
    exclude,
    from,
    ...,
    % blocks:
    analog,
    ...},
  numbers=left,
  numberstyle=\zebra{gray!20}{white}, % Don't forget to declare ZEBRA command
  showstringspaces=false,
  stepnumber=1,
  stringstyle=\color{orange},
  tabsize=2,
  % title=\lstname,
  xleftmargin=\parindent,
}

%%
% Change some of the code params:
\renewcommand{\lstlistingname}{Code Listing} % Change the listing caption
\lstset{style=custom_verilog} % By default assume all codes are verilog type


% End of code styles
% ==========================================


==> machine-learning-algos.tex <==
\subsection{Machine Learning on a Budget}
\label{sec:machine-learning}
\boxaround{
\begin{itemize}
    \item {\bf ML algos comparison:} A short subsection stating the pros and cons of different machine learning algorithms when applied to energy-constrained domain. No need fo hard numbers - just a rough estimates saying GREAT/GOOD/OK/BAD/WORST. Possible comparison {\bf table}:
        \begin{itemize}
            \item Energy
            \item Delay
            \item Accuracy
            \item How easy to tune the EDP-accuracy tradeoff
        \end{itemize}
\end{itemize}
}

As mentioned earlier, today's world is trending towards mobile computing --
according to the comScore report, people of age 18-64 spend $\approx 70\%$ of
their digital time using a mobile device \cite{comscore:2016}, and given that
the mobile devices are becoming more and more integrated with day-to-day
activities, ML algorithms are pervasively used. Applications like speech
recognition on mobile devices although used more and more often, are still
evaluated remotely because the energy budgets don't allow building a powerful ML
machine on a mobile device. Another example is handwriting recognition -- open
source NBIS library from NIST uses multi-layer perceptron for handwriting
identification and verification \cite{nist:nbis}.

When considering a ML accelerator for a mobile systems, one must consider the
trade-offs for every algorithm. Table \ref{table:ml-comparison} shows a coarse
comparison for several different design considerations (derived from
\cite{microsoft:azure}). We are not considering synthetic and ambiguous metrics
like ``run-time tunability'' or ``memory footprint'' \ajay{You have run-time
tunability in the table}. The scores given in the table are only for reference
purposes \ajay{What do you mean by for reference only?}. The ``Run-Time
Tunability'' is a custom defined metric, and represents how easy it is to tune
some of the components of the algorithm to achieve better energy-efficiency
(hardware implementation only).

\begin{table}[tbh]
    \centering
    % \vspace{-15pt}
    \caption{Machine Learning Classifiers Cheat Sheet}
    \label{table:ml-comparison}
    \vspace{-10pt}
    \begin{tabular}{lcccc}
        \toprule
        ~                   & ~                     & Energy                & Run-time      & Training                      \\
        Algorithm           & Accuracy              & Efficiency            & Tunability    & Time                              \\
        \midrule
        Logistic Regression & $\times$              & \checkmark\checkmark  & \checkmark    & \checkmark\checkmark              \\
        Random Forest       & \checkmark\checkmark  & \checkmark            & \checkmark    & \checkmark   \\
    Boosted Decision Tree   & \checkmark\checkmark  & \checkmark            & --            & \checkmark   \\
        Neural Network      & \checkmark\checkmark  & $\times$              & \checkmark    & $\times$ \\
        Averaged Perceptron & \checkmark            & $\times$              & --            & \checkmark \\
        SVM\footnotemark    & --                    & --                    & --            & -- \\
        \midrule
        Proposed Approach   & \checkmark\checkmark  & \checkmark            & \checkmark\checkmark    & --   \\
        \bottomrule
    \end{tabular}
\end{table}
\footnotetext{Depends on the choice of Kernel}


==> machine-learning-applications.tex <==
\subsection{Machine Learning Applications}
\label{sec:machine-learning-applications}
\boxaround{
\begin{itemize}
    \item {\bf Applications for ML:} A short subsection describing applications for machine learning on mobile devices. We need a list of several possible applications that are used on a daily basis
\end{itemize}
}

Machine Learning based classifiers have seen an increased deployment in a
variety of applications including speech and handwriting recognition,
photography, online shopping, and big data analysis. Today the digital world is
swaying more towards using ``smart'' machines to simplify day-to-day tasks. For
example in the field of healthcare, ML algorithms are being proposed and used
for applications like processing large amount of health data, managing hospital
admissions, predicting strokes and seizures \cite{webpage:six-applications}. In
the past decade we have also seen the ML algorithms used in education to provide
automated assessment of students' performance, online shopping to give
suggestions, and even powering ``smart'' cities. However, these applications,
being connected to the power grid, are all assumed to have virtually
``unlimited'' energy budgets. For example the work demonstrated by Le et al. in
collaboration with Google Inc. has shown a deep network that had 1 billion
trainable parameters \cite{ranzato:icml:2012}, and has shown very high accuracy
in the applications like ImageNet. However, although such machines are highly
accurate for certain applications, fail in the field of energy budgeted
computing.


==> marcia_papers.tex <==
\section{Related Work}
\label{sec:related-work}

Algorithmically, our proposed approach is based on RF classifiers \cite{breiman}. Traditionally, energy efficiency has not been considered when designing random forests, however recent work has studied learning RFs subject to test-time constraints \cite{icml2015_nan15}. This approach centers on reducing feature/sensor acquisition cost, however does not address the system energy constraints. Similar approaches to learning decision rules to minimize error subject to a budget constraint during prediction-time have been proposed\cite{Gao+Koller:NIPS11,DBLP:conf/icml/XuWC12,trapeznikov:2013b, NIPS2015_5982,ASTC_AAAI14,icml2015_nan15}. Although closely related, these approaches also ignore the energy usage and generally disregard computational cost, making them of limited use in energy constrained settings.

HMAX \cite{maashri2012accelerating},\cite{park2012fpga} based accelerator for object recognition, face identification, facial expression recognition, and action recognition. HMAX model has a hierarchal features extraction method with two stages of convolutional template matching and pooling operations. The accelerator consists of 2D systolic arrays that are dynamically configured to support different layers. Later this work was implemented on an FPGA.

Cnvlutin(CNV) \cite{albericiocnvlutin} is a value based DNN accelerator that uses a Zero-Free Neuron Array format to store the input for each layer which dynamically eliminates most ineffectual multiplications. The main focus of CNV is on the convolutional layer as it dominates execution time. The proposed CNV design is based on the state of the art DaDianNao accelerator design with improvement in performance and energy. 

EIE \cite{han2016eie}, an efficient inference engine, operates on compressed Deep Neural Network. It is a specialized accelerator designed with an array of processing elements (PEs) to perform customized sparse matrix-vector multiplication and efficiently handle weight sharing. A part of the network is stored in SRAM of a PE and it uses that part for its computation. 

Eyeriss \cite{chen2016eyeriss} is a spatial architecture based on dataflow in different layers of CNN. The dataflow is hierarchically categorized into several levels called row stationary(RS). In the new dataflow model, each row pair stays stationary to the Processing Element (PE). It increases the throughput of both convolutional and fully-connected layers and optimizes all types of data movement in the storage hierarchy.  

ISAAC \cite{shafiee2016isaac} is an in-situ analog accelerator that is similar to DaDianNao in the system organization, as it has multiple nodes/tiles but with memristor crossbar arrays in each tile. These crossbar stores dedicated a set of neuron and perform the dot-product computations. The design is easy to pipeline because outputs of the previous layer are fed to other crossbars dedicated to processing the next CNN layer, and so on. More crossbars with same weights are created to improve the throughput of a layer. 

PRIME \cite{chi2016prime} is a Processing In Memory architecture for NN that uses metal-oxide resistive random access memory (ReRAM) crossbar for dot product computation. The ReRAM main memory is designed such that a part of the memory is NN accelerator and the rest is the memory. This partition of ReRAM is dynamically reconfigured between memory ad accelerators with architecture and software support. 
Input-recycling Convolutional Array of Neurons (ICAN), is a flexible 3D compute title that implements the convolution operations used in DNNs. ICAN is efficient and supports a range of convolution layer shapes. ICAN is used along with Input Reuse Network, which is a 2D mesh-like array of registers to facilitate data reuse.

In order \cite{rahman2016efficient} to reduce the area, power and energy requirements of conventionally DNNs, they apply stochastic computing to DNNs. The goal is achieved by removing near-zero weights, applying weight scaling and state machines for activation function with an accumulator. They also propose early decision termination to save energy and increase decision speed. 
